Tableaux Modulo Theories Using Superdeduction

We propose a method that allows us to develop tableaux modulo theories using the principles of superdeduction, among which the theory is used to enrich the deduction system with new deduction rules. This method is presented in the framework of the Zenon automated theorem prover, and is applied to the set theory of the B method. This allows us to provide another prover to Atelier B, which can be used to verify B proof rules in particular. We also propose some benchmarks, in which this prover is able to automatically verify a part of the rules coming from the database maintained by Siemens IC-MOL. Finally, we describe another extension of Zenon with superdeduction, which is able to deal with any first order theory, and provide a benchmark coming from the TPTP library, which contains a large set of first order problems.

==> impl.tex <==
% $Id: impl.tex,v 1.1.1.1 2014-06-26 13:13:37 delahaye Exp $

\section{Implementation}
\label{sec:impl}

\zenon{} offers the ability to extend its core of deductive rules to match 
certain specific requirements like superdeduction. Concretely, the 
superdeduction extension of \zenon{} is an \ocaml{} file in which the 
superdeduction rules of the Figures~\ref{fig:bset-sded1} 
and~\ref{fig:bset-sded2} are implemented. This file is loaded through 
command-line options when \zenon{} is started, along with a \coq{} file 
containing the translation of the superdeduction rules.

\subsection{Handling of Metavariables}

The metavariables in the superdeduction rules are not implemented like regular 
\zenon{} metavariables. When a universal formula $\fa{}x\;P(x)$ is encountered 
by \zenon{}, the new metavariable $X$ introduced by the rule $\gamma_{\fa{}M}$ is 
linked to the universal formula. Then, when there is a potential contradiction 
such as $\lnot{}R(t,X)$, the rule $\gamma_{\fa{}inst}$ is applied in the current 
branch on the initial universal formula. In the superdeduction rules, the 
universal formulas do not appear since they are compiled in the rules. 
Consequently, the universal formulas do not appear in the proof and linking 
metavariables to them does not make sense. A solution to this is to link these 
metavariables to the antecedent formula of the rule directly. Thus, the 
instantiation will be done in the current branch from this formula.

Some superdeduction rules, as for example the rule ${a^{-1}}^*$ presented in 
Subsection~\ref{subsec:rel}, contain several metavariables. The instantiation of
these rules has to be handle specifically because \zenon{} cannot do more than
one instantiation at the same time. 
%% Therefore, we have to handle with the two 
%% instanciations in our implementation.
Let be a rule 
$R:\varphi\rightarrow{}\fa{}x\fa{}y\;P(x,y)$. Without superdeduction rules, 
the \zenon{} instantiation of the formula $\fa{}x\fa{}y\;P(x,y)$ is dealt as 
follows~:

\begin{center}
\AXC{$\fa{}x\fa{}y\;P(x,y)$}\RL{$\gamma_{\fa{}inst}$}
\UIC{$\fa{}y\;P(t_x,y)$}\RL{$\gamma_{\fa{}inst}$}
\UIC{$P(t_x,t_y)$}\DP
\end{center}

In superdeduction, in order to instanciate these two metavariables,
three rules are necessary. The compiled rule corresponding to the rule $R$ and
the instantiation rules are the following:
\begin{center}
 \begin{tabular}{c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c@{\hspace{0.5cm}}c}
   \AXC{$\varphi$}\RL{$R$}
   \UIC{$P(X,Y)$}\DP&
   \AXC{$\varphi$}\RL{$R_X$}
   \UIC{$P(t_x,Y')$}\DP&
   \AXC{$\varphi$}\RL{$R_Y$}
   \UIC{$P(X',t_y)$}\DP&
   \AXC{$\varphi$}\RL{$R_{XY}$}
   \UIC{$P(t_x,t_y)$}\DP
\end{tabular}
\end{center}
The instantiation mechanism of \zenon{} induces an order on these rules. 
Actually, if \zenon{} applies the rule $R^+_X$ then $R^+_Y$ or vice-versa, the 
last rule which can be applied is the rule $R^+_{XY}$. This step is not possible 
because the universal formulas, in which an instanciation appear (as 
$\fa{}y\;P(t_x,y)$ for the rule $R^+_X$), are hidden in the compiled rule. 
Without these formulas, \zenon{} has no information about the instantiations 
already done and then, it cannot make the two instantations at the same time. To
deal with this problem, we have to order the application of 
these rules in this way: $R^+_X$, $R^+_{XY}$ or $R^+_Y$, $R^+_{XY}$ and to 
gather the instantiation done by the first rule. In practice, we use a hash 
table which contains all the instanciations; the metavariables are linked at the
formula $\varphi$ and at the hash table reference of the last instanciation of 
the other metavariable. For instance, in the rule $R^+_X$, the metavariable $X'$
is linked at $\varphi$ and at a reference of $t_y$. Since each instanciation has
a unique reference in the hash table, a new metavariable (in our case $X'$) is 
created at each application of the rules $R^+_X$ and $R^+_Y$. After the 
application of one of these rules, \zenon{} can apply the rule $R^+_{XY}$ by 
recovering an instanciation thanks to the reference linked in a metavariable and
with the new instanciation for the other metavariable.

We illustrate this solution on the example of the Subsection~\ref{subsec:rel} 
in which the metavariables $Y$ and $Z$ are respectively instantiated by
$\epsilon_y$ and $\epsilon_z$ as follows:

$$\rootAtTop
\AXCm{\begin{array}{c}
\vdots{}\\
\odot{}
\end{array}}
\UICm{X\not\in{}p}
\AXCm{\pi}
\AXCm{\begin{array}{c}
\vdots{}\\
\odot{}
\end{array}}
\UICm{x\neq(Y,Z)}
\AXCm{\begin{array}{c}
\odot{}
\end{array}}
\UICm{p\neq{}p}\RLm{\mathrm{pred}}
\BICm{(Y,Z)\not\in{}p}\RLm{\neg{}a^{-1}}
\UICm{(Z,Y)\not\in{}p^{-1}}\RLm{\neg{}{a^{-1}}^*}
\BICm{X=(\epsilon_y,\epsilon_z),\epsilon_y\in{}a,\epsilon_z\in{}b}
\RLm{\times{}^*}
\UICm{X\in{}a\times{}b}\RLm{\subseteq{}}
\BICm{p\subseteq{}a\times{}b,x\in{}p,x\not\in{}(p^{-1})^{-1}}\DP$$

where $\pi$ is this proof tree:
$$\rootAtTop
\AXCm{\begin{array}{c}
\vdots{}\\
\odot{}
\end{array}}
\UICm{x\neq(\epsilon_y,\epsilon_z)}
\AXCm{\begin{array}{c}
\vdots{}\\
\odot{}
\end{array}}
\UICm{(\epsilon_y,\epsilon_z)\not\in{}p}
\RLm{\neg{}{a^{-1}}}
\UICm{(\epsilon_z,\epsilon_y)\not\in{}p^{-1}}
\RLm{\neg{}{a^{-1}_{YZ}}^*}
\BICm{x\neq(\epsilon_y,Z')}
\AXCm{\begin{array}{c}
\vdots{}\\
\odot{}
\end{array}}
\UICm{(Z',\epsilon_y)\not\in{}p^{-1}}
\RLm{\neg{}{a^{-1}_Y}^*}
\BICm{x\neq(Y,Z)}\DP
$$

%% arbre complet
%% $$\rootAtTop
%% \AXCm{\begin{array}{c}
%% \vdots{}\\
%% \odot{}
%% \end{array}}
%% \UICm{X\not\in{}p}
%% \AXCm{\begin{array}{c}
%% \vdots{}\\
%% \odot{}
%% \end{array}}
%% \UICm{x\neq(\epsilon_y,\epsilon_z)}
%% \AXCm{\begin{array}{c}
%% \vdots{}\\
%% \odot{}
%% \end{array}}
%% \UICm{(\epsilon_y,\epsilon_z)\not\in{}p}
%% \RLm{\neg{}{a^{-1}}}
%% \UICm{(\epsilon_z,\epsilon_y)\not\in{}p^{-1}}
%% \RLm{\neg{}{a^{-1}_{YZ}}^*}
%% \BICm{x\neq(\epsilon_y,Z')}
%% \AXCm{\begin{array}{c}
%% \vdots{}\\
%% \odot{}
%% \end{array}}
%% \UICm{(Z',\epsilon_y)\not\in{}p^{-1}}
%% \RLm{\neg{}{a^{-1}_Y}^*}
%% \BICm{x\neq(Y,Z)}
%% \AXCm{\begin{array}{c}
%% \vdots{}\\
%% \odot{}
%% \end{array}}
%% \UICm{x\neq(Y,Z)}
%% \AXCm{\begin{array}{c}
%% \odot{}
%% \end{array}}
%% \UICm{p\neq{}p}\RLm{\mathrm{pred}}
%% \BICm{(Y,Z)\not\in{}p}\RLm{\neg{}a^{-1}}
%% \UICm{(Z,Y)\not\in{}p^{-1}}\RLm{\neg{}{a^{-1}}^*}
%% \BICm{X=(\epsilon_y,\epsilon_z),\epsilon_y\in{}a,\epsilon_z\in{}b}
%% \RLm{\times{}^*}
%% \UICm{X\in{}a\times{}b}\RLm{\subseteq{}}
%% \BICm{p\subseteq{}a\times{}b,x\in{}p,x\not\in{}(p^{-1})^{-1}}\DP$$

%% $$\rootAtTop
%% \inferrule* [Right=$\subseteq$]
%%            { p\subseteq{}a\times{}b,x\in{}p,x\not\in{}(p^{-1})^{-1} }
%%            { \inferrule*
%%              { X\not\in{}p }
%%              { \odot }
%%              \\ 
%%              \inferrule* [Right=$\times{}^*$]
%%                         { X\in{}a\times{}b }
%%                         { 
%%                           \inferrule*
%%                           { X=(\epsilon_y,\epsilon_z),\epsilon_y\in{}a,\epsilon_z\in{}b}
%%                           { 
%%                             \inferrule*[Right=$\neg{}{a^{-1}_Y}^*$]
%%                             {x\neq(Y,Z)}
%%                             {(Z',\epsilon_y)\not\in{}p^{-1}}
%%                             \\
%%                             (Z,Y)\not\in{}p^{-1}
%%                           }
%%  }
%%            }
%% $$


\subsection{Producing \coq{} Proofs}

Since we have extended the proof system of \zenon{}, we must extend the \coq{}
proofs generation. For each superdeduction rule of the 
Figures~\ref{fig:bset-sded1} and~\ref{fig:bset-sded2}, we have 
a \coq{} lemma corresponding to the translation of the rule. These lemmas are
encoded in a shallow embedding of the \bmth{} set theory in \coq{}.  
At \siemens{}, a deep embedding of the \bmth{} set theory in \coq{}~\cite{JA11} 
has
been developped. Eventually, we would like to translate the \coq{} proofs 
generated by \zenon{} into this embedding in order to have the correction of
our approach with regard to the \bbook{}.

A difference with the \coq{} proofs producing of \zenon{} without superdeduction
can be observed when two different formulas generate the same Hilbert's 
operator. For example, if we have the following proof extract:

$$\rootAtTop
\AXCm{\begin{array}{c}
\vdots{}\\
\odot{}
\end{array}}
\UICm{\lnot{}(\epsilon_x\in{}a\Rightarrow{}\epsilon_x\in{}b)}\RLm{\lnot{}\fa{}}
\UICm{\epsilon_x\in{}a,\epsilon_x\notin{}b}\RLm{\lnot{}\pow}
\UICm{a\notin{}\pow(b),\lnot{}\fa{}x.(x\in{}a\Rightarrow{}x\in{}b),\Delta}\DP$$

where $\epsilon_x=\epsilon(x).\lnot{}(x\in{}a\Rightarrow{}x\in{}b)$.

Without superdeduction, \zenon{} exploit each $\delta$ rule once per formula in
a proof. Thus, it does not generate two times the same Hilbert's operator.
In our example, a problem
appears during the \coq{} proof check because in this proof, the same term is
inserted two times. More precisely, the two following rules will
introduce the same term, at the time of the introductions of both
{\verb=forall=}:

{\small
\begin{lstlisting}[language=Coq,basicstyle=\footnotesize,mathescape]
Lemma zenon_notall : forall (T : Type) (P : T -> Prop),
  (forall z : T, (~(P z) -> False)) -> 
  (~(forall x : T, (P x)) -> False).
\end{lstlisting}}

{\small
\begin{lstlisting}[language=Coq,basicstyle=\footnotesize,mathescape]
Lemma zenon_B_notpow : forall a b c : U,
  (forall x : U, (x $\in$ a -> x $\notin$ b -> False)) ->
  ((a $\notin$ $\pow($b$)$) -> False).
\end{lstlisting}}

To solve this 
problem, we have to give a fresh name at this term when it is introduced for the
second time. The proof is then correct since the formulas with the first 
Hilbert's operator name will be already present in the proof.


